VisTaNet: Attention Guided Deep Fusion for Surface Roughness Classification

Human texture perception is a weighted average of multi-sensory inputs: visual and tactile. While the visual sensing mechanism extracts global features, the tactile mechanism complements it by extracting local features. The lack of coupled visuotactile datasets in the literature is a challenge for studying multimodal fusion strategies analogous to human texture perception. This paper presents a visual dataset that augments an existing tactile dataset. We propose a novel deep fusion architecture that fuses visual and tactile data using four types of fusion strategies: summation, concatenation, max-pooling, and attention. Our model shows significant performance improvements (97.22%) in surface roughness classification accuracy over tactile only (SVM - 92.60%) and visual only (FENet-50 - 85.01%) architectures. Among the several fusion techniques, attention-guided architecture results in better classification accuracy. Our study shows that analogous to human texture perception, the proposed model chooses a weighted combination of the two modalities (visual and tactile), thus resulting in higher surface roughness classification accuracy; and it chooses to maximize the weightage of the tactile modality where the visual modality fails and vice-versa.

==> sections/intro.tex <==
\section{Introduction}
% importance of surface texture and its contextual study:




Textures are psychophysical, not physical. They are composed of atleast four prominent psychophysical dimensions that are perceived as roughness/smoothness, hardness/softness, sticky/slippery, and coldness/warmness \cite{okamoto2012psychophysical}. Texture plays an important role in the industrial setting because it correlates to the feel of the product, material finish, and adhesion. Roughness is the texture dimension that has proven reliable over time when attempting to understand the effects of corrosion, cracks, irregularities, friction, and wear and tear on a finished product. Furthermore, roughness can be represented in 3-dimension (lay, spacing, and depth) \cite{leung2001representing, ojala2001texture}. Lay is the direction of dominant pattern of texture on the surface of a finished product \cite{iso_21920_1_2021}, which gives an overall measure of the final product's visual and tactile characteristics.

Robots are being employed in industries for trimming, drilling, and machining, despite the stiffness constraints of articulated robotic arms. In line with this, using a feedback sensing element simultaneously for assessing finished surface texture can be advantageous \cite{jiang2022robotic} in applications such as surface castings \cite{tsai1999surface}, milling, and turning.

% What is tecture perception?
Textural sensors and feedback systems are mostly inspired from human texture perception. The senses of vision and touch combined to form a person's texture perception \cite{yoshioka2007texture} and touch-based texture perception develops very early compared to vision \cite{FIELD2008364}. Although vision-based textural studies are presented \cite{julesz1981textons}, it is not the same as actual texture perception. While vision and touch perform well for macro-roughness, touch performs better for micro-roughness \cite{heller1989texture}. Neither vision nor touch, as demonstrated in an early study \cite{lederman1986perception, ernst2002humans}, are solely responsible for spatial acuity or the perception of roughness. In other words, different sensory signalling processes are interconnected and influenced by one another during perception. While vision accounts for the 2-dimensions of roughness (lay and spacing), tactile may account for all the three dimension of roughness.

% literature on methods used for classification of textures
Several methods emerged recently for  texture classification. Although the task seems trivial for humans, it remains a major challenge for machine vision. Visual texture classification aims to identify if a given image patch or image belongs to a specific texture category. The conventional methods have used various hand-crafted feature-based approaches such as wavelet packet signatures \cite{laine1993texture, arivazhagan2003texture, dong2011wavelet}, rotation- and scale-invariant Gabor features \cite{bianconi2007evaluation, riaz2013texture} %, texture spectrum \cite{wang1990texture}, Neighboring Gray Level Dependence Matrix (NGLDM) \cite{sun1983neighboring} and also simple model based method \cite{kashyap1986model}
for classification. Singular Value Decomposition (SVD) \cite{selvan2007svd}, Support Vector Machine (SVM) \cite{kim2002support}, local binary pattern (LBP) \cite{ojala2000gray, ojala2002multiresolution, guo2010completed, banerji2011novel}, %energies of image sub-bands \cite{smith1994transform}, 
and Convolutional Neural Network (CNN) \cite{fujieda2018wavelet, andrearczyk2016using} based methods %, Griffin and Lillholm image features \cite{crosier2010using}, spectral histogram \cite{liu2003texture}, and a simple bayesian classifier \cite{tsai1999surface} 
are widely used. A review of methods for image-based texture classification is presented in \cite{armi2019texture}.

% some new novel methods that fuse tactile and visual information
Prior studies decode texture using tactile sensing mechanisms such as the GelSight \cite{yuan2017gelsight} or simply surface classification using a whisker sensor \cite{wolfe2008texture, jadhav2010texture, hipp2006texture}. A naive accelerometer-based whisker sensor for terrain classification is presented in \cite{giguere2009surface, dallaire2014autonomous}. A few studies used maximum covariance analysis to combine both visual and tactile sensing for texture classification \cite{luo2018vitac, kroemer2011learning}. The visual sensing mechanism can act as a global predictor and the tactile sensing can complement the vision system by providing local information about surface texture. Due to the lack of coherent visuo-tactile datasets, none of these studies explored how these two modalities of texture can be combined for accurate surface roughness classification. 

\begin{figure*}[ht]
\centering
\includegraphics[width=\textwidth]{Block_diagram_architecture.png}
\caption{\textit{Overview of the visuo-tactile dataset pipeline and the proposed network architecture.} The visual texture dataset pipeline provides the outline for processing the captured images from the specimen. The visual and tactile streams extract features from corresponding visual and tactile data. The feature fusion module combines the two features passing them to the classifier downstream. The classifier module comprises a stack of two fully-connected layers followed by an 18-class softmax layer which predicts the texture roughness.}
\label{fig:mainfigure}
\end{figure*}

% GOAL:
In this paper, we investigate methods to improve the accuracy of surface roughness classification using deep-learning models. Existing literature suggests that human texture understanding can be interpreted as a weighted average of multi-sensory inputs. Achieving similar performance in robots would require a coherent visuotactile dataset. To this end, we propose a visual dataset that augments an existing tactile dataset. Further, we present a novel attention-guided deep fusion architecture that combines the visual and tactile modalities using a weighted average. Our model shows significant performance improvements over \textit{tactile only} \& \textit{visual only} architectures for surface roughness classification. Finally, we perform an ablation study comparing various fusion strategies for combining visual and tactile features showing that the attention-based fusion strategy offers the best performance improvements.
